Shape of synth to come: Why we should use synthetic data for English surface realization

The Surface Realization Shared Tasks of 2018 and 2019 were Natural Language Generation shared tasks with the goal of exploring approaches to surface realization from Universal-Dependency-like trees to surface strings for several languages. In the 2018 shared task there was very little difference in the absolute performance of systems trained with and without additional, synthetically created data, and a new rule prohibiting the use of synthetic data was introduced for the 2019 shared task. Contrary to the findings of the 2018 shared task, we show, in experiments on the English 2018 dataset, that the use of synthetic data can have a substantial positive effect - an improvement of almost 8 BLEU points for a previously state-of-the-art system. We analyse the effects of synthetic data, and we argue that its use should be encouraged rather than prohibited so that future research efforts continue to explore systems that can take advantage of such data.

==> tex_files/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Topic - The task itself
The shallow task of the surface realization shared task appears to be a relatively straightforward problem \citep{first_surface_realization_shared_task, mulit_surface_realization_2018, second_surface_realization_2019}. 
%
Given a tree of lemmas a system has to restore the original word order of the sentence and inflect its lemmas, see Figure \ref{fig:surface_realization_example}. 
% Question - How to get the best performance 
However, systems struggle to solve the problem, often failing to recover the original sentence.
% Significance - More complex forms of the task that might be more useful in practice
Improved performance would facilitate investigation of more complex versions of the shallow task, such as the deep task in which function words are pruned from the tree, which may be of more practical use in pipeline natural language generation (NLG) systems \citep{moryossef-etal-2019-step, elder-etal-2019-designing, castro-ferreira-etal-2019-neural}. 
% Improved performance would facilitate investigation of more complex versions of this problem,


% More significance - Ehud Reiter and the quality
Ehud Reiter is a frequent critic of neural NLG approaches\footnote{\url{https://ehudreiter.com/}}, emphasising that quality and reliability are at the core of production ready NLG systems.

% Preamble / claim(?) - Use of synthetic data
In this paper we explore the use of synthetic data for the shallow task.
%
Synthetic data is created by taking an unlabelled sentence, running it through an open source universal dependency parser\footnote{A number of these exist; \url{https://github.com/stanfordnlp/stanfordnlp} \url{http://lindat.mff.cuni.cz/services/udpipe/}} and transforming the result into the input representation.

% Claim - Extra data is really important for this task and the quality
Unlike in the shared task of 2018, where a system trained with synthetic data performed roughly the same as a system trained on the original dataset \citep{elder_srst_2018, king_white_srst_2018}, we find it leads to a large improvement in performance.
% Evidence - Scores are much higher
The state-of-the-art on the dataset is 72.67 BLEU-4 score \citep{yu-etal-2019-head}, our system achieves a similar result of 72.3, which improves to 80.1 with the use of synthetic data.
% Reason - Analyse what the extra data helps to improve
In section \ref{sec:results} we analyse the ways in which synthetic data helps to improve performance.
% Probably not necessary but could mention the other fields like text classification / sequence labelling (unsupervised language model pretraining) and machine translation (synthetic data using back translation)

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/acl_srst_paper.pdf}
    \caption{Input tree for the sentence \emph{This story comes from the AP:}   \emph{(Will be re-done in google drawings)}}
    \label{fig:surface_realization_example}
\end{figure}

% Preamble / Claim - Not allowed to use additional data this year
% Then we talk about the question of additional data
This result is important for a further reason - the 2019 shared task introduced a new rule which banned the use of synthetic data in order to make the results of different systems more comparable.
% s that by having all systems train on the same set of data results would be more comparable. 
%
However, systems designed with smaller datasets in mind might not scale to the use of synthetic data, hence this new rule may produce results which could be misleading for future research directions.

For instance, this year's clear winning system by \citet{ims_srst_2019} used tree-structured long short-term memory (LSTM) networks \citep{tai_tree_lstm_2015}.
%
In general tree LSTMs can be slow and difficult to train\footnote{\url{https://github.com/dasguptar/treelstm.pytorch/issues/6}}.
%
\citet{graphAMR_ACL2018} utilized a variant of the tree LSTM in a similar NLG task, converting abstract meaning representation (AMR) graphs to text.
%
Following the state-of-the-art system \citep{neural_amr_konstas_ACL_2017}, which used standard LSTMs, \citeauthor{graphAMR_ACL2018} augmented their training with synthetic data.
%
Their system outperformed \citeauthor{neural_amr_konstas_ACL_2017} at equivalent levels of additional training sentences.
%
However, their system was unable to scale up to the 20,000,000 sentences used by the best \citeauthor{neural_amr_konstas_ACL_2017} system and ultimately did not outperform it\footnote{\citeauthor{graphAMR_ACL2018}'s best system achieved 33.0 bleu score with 2 million additional sentences vs. \citeauthor{neural_amr_konstas_ACL_2017}'s 32.3 with 2 million and 33.8 with 20 million, the best overall system}.

Essentially, if using synthetic data contributes to producing the highest quality outputs, then we ought to ensure we are designing systems that can take advantage of synthetic data.



% Say something about the different languages. That although we test only on english the system is designed to take input in the form of UD trees, which are universal. 
